Binary Image Skeletonization Using 2-Stage U-Net

Object Skeletonization is the process of extracting skeletal, line-like representations of shapes. It provides a very useful tool for geometric shape understanding and minimal shape representation. It also has a wide variety of applications, most notably in anatomical research and activity detection. Several mathematical algorithmic approaches have been developed to solve this problem, and some of them have been proven quite robust. However, a lesser amount of attention has been invested into deep learning solutions for it. In this paper, we use a 2-stage variant of the famous U-Net architecture to split the problem space into two sub-problems: shape minimization and corrective skeleton thinning. Our model produces results that are visually much better than the baseline SkelNetOn model. We propose a new metric, M-CCORR, based on normalized correlation coefficients as an alternative to F1 for this challenge as it solves the problem of class imbalance, managing to recognize skeleton similarity without suffering from F1's over-sensitivity to pixel-shifts.

==> Setup.tex <==
\section{Setup}
\subsection{End-to-End Audio Expert}
This audio expert takes the audio features generated by the Audio Generator described earlier and gets independently trained on classifying the 10 genres. 
\subsection{End-to-End Spectrogram Expert}
A CNN of that takes the photos of the spectrogram graphs of the audio and gets independently trained on them to classify the 10 genres. 
\subsection{Flat MoE}
In this architecture, we concatenate two types of features: the Audio Generator features and the Spectrogram Expert output features. We extract the Spectrogram Expert output features by taking the output of the last layer before the fully connected classifying layers, which should typically contain more meaningful features. Both of the audio and spectrogram features get concatenated and fed into a Terminal Expert that is trained on classifying their corresponding genres. 
\begin{figure}[H]
\centering
\includegraphics[width=0.4\textwidth]{images/moe_flat.eps}
\caption{F-MoE with Flat Classes Architecture}
\end{figure}
\subsection{Hierarchical MoE}
In this architecture, unlike the flat architecture, we replace the Terminal Expert with a hierarchical mixture of experts that are designed based on our problem-space division. First, there is a super-classifier, which determines to which super-class an image belongs to. Based on the super-classifier output, the sub-classifier experts are enabled, while each is only specialized in classifying its own cluster of labels. We divided the labels hierarchically based on the similarity levels between the genres since grouping similar genres under one cluster makes it less confusing for the classifier if it is trained on that cluster only. Then, we combine the output of the sub-classifiers to get the final label belong to the 10 atomic genres. 
\begin{figure}[H]
\centering
\includegraphics[width=0.7\textwidth]{images/moe_hierarichal.eps}
\caption{H-MoE with Hierarchical Classes Architecture}
\end{figure}

==> abstract.tex <==
Owing to the constant growth of the music industry, classifying songs by their genre has become increasingly relevant to many applications to provide a variety of features often demanded by end-users. In this paper, we explore a relatively new approach for the said problem by utilizing the Hierarchical Mixture of Experts approach on song genres. Our method works by delegating different types of features to their dedicated, specialized experts whose extracted features are fused together to be fed to a set of terminal classifiers for the final predictions. Another key aspect of this approach is grouping classes into a hierarchy thereof in order to split the classification process on multiple stages. Our results have shown a promising improvement on citations following a similar approach.


==> includes.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{booktabs}
\usepackage[english]{babel}
\usepackage{ifpdf, newtxtext,newtxmath} 
\usepackage{natbib}
\usepackage{wrapfig}
\usepackage{longtable}
\usepackage{graphicx}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage[table,xcdraw]{xcolor}
\usepackage[export]{adjustbox}
\usepackage[rightcaption]{sidecap}
\usepackage{subfig}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
\usepackage{float}
\usepackage{multirow}
\usepackage[table,xcdraw]{xcolor}
\usepackage[export]{adjustbox}
\usepackage[rightcaption]{sidecap}
\usepackage{subfig}
\usepackage{subcaption}
\usepackage{array, dcolumn,multirow,hevea,abstract,hanging,fancyhdr}
% change next 3 lines each issue
\newcommand{\jref}{http://journal.sjdm.org/vol16.1.html}
\newcommand{\jhead}{https://github.com/Oschart/MoE-Music-Classifier}
\newcommand{\jdate}{\today}
\topmargin=-.3in \oddsidemargin=.3in \evensidemargin=.3in \textheight=9in \textwidth=6in
\pagestyle{fancy} 
\fancyhead[L]{\protect\small \href{\jref}{\jhead}, \jdate}
\fancyhead[R]{\protect\small MGC Using MoE} % replace with running head
\fancypagestyle{firstpage}{%
 \lhead{\protect\small \href{\jref}{\jhead}, \jdate}
 \rhead{}
}
\usepackage[labelfont=sc,textfont=sf]{caption}
\usepackage[hyperfootnotes=false,breaklinks=true]{hyperref} % was dvipdfmx

\urlstyle{rm}
\usepackage[hyphenbreaks]{breakurl}
% DO NOT USE ADDITIONAL PACKAGES unless you make sure they work with Hevea.
% You may define new commands, but these may cause other troubles, so try to avoid it.

% FOR BIBTEX USERS (Bibtex is not recommended, but we can use it):
% \usepackage{natbib} % must come afer hypperref
% in references: \bibliographystyle{apalike3} \setlength{\bibsep}{0pt} \bibliography{WHATEVER}
% download http://journal.sjdm.org/apalike3.bst
\usepackage{booktabs} % \toprule \midrule \bottomrule \cmidrule(lr){a-b}
% define centered and ragged columns:
\newcolumntype{L}[1]{>{\raggedright\arraybackslash }p{#1}} % can use m{}
\newcolumntype{C}[1]{>{\centering\arraybackslash }p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash }p{#1}}
\newcolumntype{d}[1]{D{.}{.}{#1}} % d{3.2} for 3 places on l, 2 on r
\newcommand{\mc}{\multicolumn}
\setlength\tabcolsep{1mm}
\setlength\columnsep{5mm}
\setlength\abovecaptionskip{1ex}
\setlength\belowcaptionskip{.5ex}
\setlength\belowbottomsep{.3ex}
\setlength\lightrulewidth{.04em}
\renewcommand\arraystretch{1.2}
\renewcommand{\topfraction}{1}
\renewcommand{\textfraction}{0}
\renewcommand{\floatpagefraction}{.9}
% \renewcommand{\baselinestretch}{1.00} \large\normalsize % for fixing spaces
\widowpenalty=1000
\clubpenalty=1000
\setlength{\parskip}{0ex}
\let\tempone\itemize
\let\temptwo\enditemize
\let\tempthree\enumerate
\let\tempfour\endenumerate
\renewenvironment{itemize}{\tempone\setlength{\itemsep}{0pt}}{\temptwo}
\renewenvironment{enumerate}{\tempthree\setlength{\itemsep}{0pt}}{\tempfour}

